Publication Bias: A Detailed Analysis of Experiments Published in ESEM

Background: Publication bias is the failure to publish the results of a study based on the direction or strength of the study findings. The existence of publication bias is firmly established in areas like medical research. Recent research suggests the existence of publication bias in Software Engineering. Aims: Finding out whether experiments published in the International Workshop on Empirical Software Engineering and Measurement (ESEM) are affected by publication bias. Method: We review experiments published in ESEM. We also survey with experimental researchers to triangulate our findings. Results: ESEM experiments do not define hypotheses and frequently perform multiple testing. One-tailed tests have a slightly higher rate of achieving statistically significant results. We could not find other practices associated with publication bias. Conclusions: Our results provide a more encouraging perspective of SE research than previous research: (1) ESEM publications do not seem to be strongly affected by biases and (2) we identify some practices that could be associated with p-hacking, but it is more likely that they are related to the conduction of exploratory research.

==> dotgraph/nodes_and_ranks <==
{rank=same; "Research hypotheses definition"; "Analytical definition of statistical hypotheses"; "Tail definition"; "Relationship between research hypotheses and statistical hypotheses";}
{rank = same; "Does not apply to some study types";"Research hypothesis is self-evident";"Decision cannot be made at design time";"Research hypothesis is not used";"H1 can be defined in prose";"Effect direction can be inferred from hypothesis definition";"Effect direction is self-evident";"Apply always the same strategy";"Do not take into consideration";"Research questions can be answered using non statistical techniques (e.g., deduction)";"Research questions cannot be always translated to statistical hypotheses";}
{rank = same; "Case studies";"Exploratory studies";"An improvement over the previous technology (/control) is expected";"Adding research hypotheses implies some cognitive overhead";"Use Research Questions instead";"Surveys";"Research hypothesis can be inferred from the study context";"Non-experimental empirical studies";"Deferred until experiment execution";"Use 2-tailed test by default";"Use 1-tailed test by default";"Use well defined tests";}

"Research hypotheses definition" [label = "Research hypotheses definition"];
"Analytical definition of statistical hypotheses" [label = "Analytical definition of\nstatistical hypotheses"];
"Tail definition" [label = "Tail definition"];
"Relationship between research hypotheses and statistical hypotheses" [label = "Relationship between research\nhypotheses and statistical hypotheses"];
"Does not apply to some study types" [label = "Does not apply\nto some study types"];
"Research hypothesis is self-evident" [label = "Research hypothesis is\nself-evident"];
"Decision cannot be made at design time" [label = "Decision cannot be\nmade at design time"];
"Research hypothesis is not used" [label = "Research hypotheses are\nnot used"];
"H1 can be defined in prose" [label = "H1 can be\ndefined in prose"];
"Effect direction can be inferred from hypothesis definition" [label = "Effect direction can be inferred\nfrom hypothesis definition"];
"Effect direction is self-evident" [label = "Effect direction is self-evident"];
"Apply always the same strategy" [label = "Apply always the\nsame strategy"];
"Do not take into consideration" [label = "Do not take\ninto consideration"];
"Research questions can be answered using non statistical techniques (e.g., deduction)" [label = "Research questions can be answered\nusing non statistical techniques (e.g., deduction)"];
"Research questions cannot be always translated to statistical hypotheses" [label = "Research questions cannot be always\ntranslated to statistical hypotheses"];
"Case studies" [label = "Case studies"];
"Exploratory studies" [label = "Exploratory studies"];
"An improvement over the previous technology (/control) is expected" [label = "An improvement over the previous\ntechnology (/control) is expected"];
"Adding research hypotheses implies some cognitive overhead" [label = "Adding research hypotheses\nimplies some cognitive overhead"];
"Use Research Questions instead" [label = "Use Research Questions\ninstead"];
"Surveys" [label = "Surveys"];
"Research hypothesis can be inferred from the study context" [label = "Research hypothesis can be inferred\nfrom the study context"];
"Non-experimental empirical studies" [label = "Non-experimental empirical studies"];
"Deferred until experiment execution" [label = "Deferred until experiment\nexecution"];
"Use 2-tailed test by default" [label = "Use 2-tailed test\nby default"];
"Use 1-tailed test by default" [label = "Use 1-tailed test\nby default"];
"Use well defined tests" [label = "Use well defined\ntests"];

==> tex-files/discussion.tex <==
\section{Discussion}\label{sec:discussion}

La Tabla~\ref{tab:summary_results} muestra un resumen de los resultados obtenidos en la revisión de literatura y el survey de experimentadores en SE. En general, los resultados son bastante congruentes, con pocas excepciones.

\input{tex-files/tables/table-discussion}

\subsection{Ausencia o falta de relación entre hipótesis de investigación e hipótesis estadística}

La revisión de literatura ha permitido confirmar que sólo una minoría de experimentos definen hipótesis estadísticas y el tipo de cola de los tests. En contrapartida, la mayoría de los investigadores indican que si utilizan estos conceptos en sus estudios. En este caso, nos encontramos antes una evidente contradicción, pero ésta es perfectamente explicable si atendemos a los comentarios de los mismos investigadores. Probablemente, lo que los investigadores quieren afirmar es que \textit{en una situación ideal}, las hipótesis y los tipos de colas \textit{deberían ser especificados}. \textit{En la práctica}, sin embargo, ello no es posible, por tres motivos:

\begin{itemize}
\item \textbf{Existe un desconocimiento los procesos que operan en IS}, que impide conocer los tipos de cola a aplicar. Nos atreveríamos a decir que este mismo desconocimiento se extiende a las variables independientes y dependientes relevantes.
\item Derivado de lo anterior, \textbf{una gran parte de la investigación realizada en IS es de carácter exploratorio}. La investigación exploratoria consiste en \cite{pmid24844265} \textit{small and flexible experiments using different methodologies [that] may or may not employ inferential statistics. Exploratory studies are often driven by a series of hypotheses that are either loosely articulated or that evolve over the course of sequential experiments}. Las hipótesis estadísticas \textit{a priori}, como muy bien indican los investigadores, no son particularmente útiles para experimentos exploratorios. 
\item Las preguntas de investigación se utilizan frecuentemente a modo de hipótesis de investigación. En muchas ocasiones (probablemente, de nuevo en experimentos exploratorios) los investigadores indican que no resulta sencillo transformar las preguntas de investigación en hipótesis estadísticas, aunque esto no se observa en los reportes experimentales; el número de experimentos que compagina hipótesis estadísticas y research questions es considerable.
\end{itemize}

\subsection{Uso arbitrario de tests 1-tailed o 2-tailed}

La revisión de literatura no ha permitido identificar ninguna práctica cuestionable. Como única excepción, existe una tendencia a no especificar el tipo de cola en tests ''complejos'', tales como ANOVA o Kruskal-Wallis. No obstante, la imposibilidad de identificar prácticas cuestionables se debe principalmente a información ausente en los reportes experimentales, e.g., el tipo de cola de los tests. Cuando preguntamos a los investigadores, la situación se clarifica:

\begin{itemize}
\item Los investigadores muestran cierta preferencia por los tests de 2 colas, ya que son más adecuados en situaciones de ignorancia acerca de la direccionalidad de los efectos.  
\item Los investigadores realizan cambios, aunque no muy frecuentemente, en los tipos de cola de los tests. \textbf{El cambio más frecuente es de 2-colas a 1-cola, lo que trae aparejando en algunas ocasiones la obtención de resultados significativos}. Se trata, probablemente, de una instancia de p-hacking.
\item Los investigadores no conocen bien el tipo de cola asociado a tests sencillos, como ANOVA, Kruskal-Wallis o $\chi^2$. Ello explica por qué los reportes experimentales no especifican el tipo de cola. Adicionalmente, en varias ocasiones, \textbf{las explicaciones de los investigadores son cuestionables desde el punto de vista de su corrección estadística}. Todo ello apunta a carencias en la formación estadística de los investigadores.
\end{itemize}

\subsection{Asociación incorrecta de las técnicas estadísticas y pruebas de hipótesis}

Al igual que en el caso anterior, la revisión de literatura no ha puesto de manifiesto prácticas dudosas. Sin embargo, los investigadores han sido muy francos en sus comentarios, aunque éstos no se alineen con la práctica ortodoxa; una cantidad sustancial de investigadores afirma \textbf{haber utilizado distintos tipos de tests durante el análisis estadístico}, lo cual sólo puede interpretarse como un fenómeno de p-hacking. 
